On Inter-dataset Code Duplication and Data Leakage in Large Language Models

Motivation. Large language models (LLMs) have exhibited remarkable proficiency in diverse software engineering (SE) tasks. Handling such tasks typically involves acquiring foundational coding knowledge on large, general-purpose datasets during a pre-training phase, and subsequently refining on smaller, task-specific datasets as part of a fine-tuning phase. Problem statement. While intra-dataset code duplication examines the intersection between the training and test splits within a given dataset and has been addressed in prior research, inter-dataset code duplication, which gauges the overlap between different datasets, remains largely unexplored. If this phenomenon exists, it could compromise the integrity of LLM evaluations because of the inclusion of fine-tuning test samples that were already encountered during pre-training, resulting in inflated performance metrics. Contribution. This paper explores the phenomenon of inter-dataset code duplication and its impact on evaluating LLMs across diverse SE tasks. Study design. We conduct an empirical study using the CodeSearchNet dataset (CSN), a widely adopted pre-training dataset, and five fine-tuning datasets used for various se tasks. We first identify the intersection between the pre-training and fine-tuning datasets using a deduplication process. Next, we pre-train two versions of LLMs using a subset of CSN: one leaky LLM and one non-leaky LLM. Finally, we fine-tune both models and compare their performances using leaky fine-tuning test samples. Results. Our findings reveal a potential threat to the evaluation of LLMs across multiple SE tasks, stemming from the inter-dataset code duplication phenomenon. We also demonstrate that this threat is accentuated by the chosen fine-tuning technique. Furthermore, we provide evidence that open-source models could be affected by inter-dataset duplication.

==> contents/appendices.tex <==

\clearpage
\appendices
\section{Layer-wise performances}


\begin{table*}[t]
\caption{Average layer-wise performances of \unixcoder{} and \graphcodebert{} for the task of code search.}
\label{tab:performancecodesearchlayer}
    \centering
\scalebox{0.8}{
\begin{tabular}{lccccc}
\toprule
        Model &  Layer &   Biased group &  Unbiased group &  Performance &  Difference \\
\hline
\graphcodebert{} &      3 & 89.16 &   88.79 & 88.84 &  0.37 \\
\graphcodebert{} &      4 & 89.28 &   88.77 & 88.83 &  0.51 \\
\graphcodebert{} &      2 & 89.26 &   88.76 & 88.83 &  0.50 \\
\graphcodebert{} &      1 & 89.31 &   88.69 & 88.77 &  0.62 \\
\graphcodebert{} &      5 & 89.40 &   88.64 & 88.74 &  0.76 \\
\graphcodebert{} &      6 & 89.40 &   88.50 & 88.61 &  0.90 \\
\graphcodebert{} &      7 & 89.10 &   88.41 & 88.50 &  0.69 \\
\graphcodebert{} &      8 & 89.03 &   88.28 & 88.37 &  0.75 \\
\graphcodebert{} &      9 & 88.89 &   88.11 & 88.21 &  0.78 \\
\graphcodebert{} &     10 & 88.78 &   87.94 & 88.05 &  0.84 \\
\graphcodebert{} &     11 & 88.11 &   86.92 & 87.07 &  1.20 \\
    \unixcoder{} &      1 & 82.47 &   81.00 & 81.19 &  1.47 \\
    \unixcoder{} &      2 & 82.44 &   80.79 & 81.00 &  1.65 \\
    \unixcoder{} &      3 & 82.44 &   80.66 & 80.89 &  1.78 \\
    \unixcoder{} &      4 & 82.58 &   80.63 & 80.88 &  1.95 \\
    \unixcoder{} &      5 & 82.59 &   80.60 & 80.86 &  1.99 \\
    \unixcoder{} &      6 & 82.45 &   80.58 & 80.82 &  1.87 \\
    \unixcoder{} &      7 & 82.63 &   80.43 & 80.72 &  2.20 \\
    \unixcoder{} &      8 & 82.39 &   79.98 & 80.29 &  2.41 \\
    \unixcoder{} &      9 & 81.77 &   79.50 & 79.79 &  2.27 \\
    \unixcoder{} &     10 & 81.09 &   78.76 & 79.06 &  2.32 \\
    \unixcoder{} &     11 & 79.06 &   76.71 & 77.01 &  2.35 \\
\bottomrule
\end{tabular}
}
\end{table*}





==> contents/related.tex <==


\section{Related work}
\label{sec:related}


In this section, we examine literature related to this study, categorized into three groups: code clone detection, code duplication within GitHub, and the impact of code duplication on ML models.

\subsection{Code clone detection}
In the code clone literature, various types of code clones are identified~\cite{roy2007survey,sajnani2016sourcerercc,golubev2021nature}. Type-1 clones involve identical code snippets with differences in spaces, comments, whitespaces, or layouts. Type-2 clones are syntactically equivalent fragments with variations in identifiers, literals, and types, along with Type-1 differences. Type-3 clones encompass all changes found in Type-1 and Type-2 clones, with additional modifications like altered, added, or removed statements. Finally, Type-4 clones represent snippets that share functionality but have different syntax.


Code clone detection tools employ the concept of \textit{similarity} to discern whether two code fragments are clones or not~\cite{zakeri2023systematic}. These tools can be broadly categorized into six groups based on how they compute similarities~\cite{zakeri2023systematic,chen2022definition}. Text-based techniques treat code as raw strings and compare them directly; NICAD~\cite{cordy2011nicad} is a prominent example in this group. Token-based approaches involve tokenizing code fragments, and similarity is typically measured as the overlap between token sequences. SourcererCC~\cite{sajnani2016sourcerercc} belongs to this group. Tree-based tools use the ASTs or parse trees to compute similarity. For instance, DECKARD~\cite{jiang2007deckard} falls into this group and employs a tree edit distance metric. Graph-based techniques leverage program dependency graphs. For example, CCSharp, a C\# clone detector, falls into this category~\cite{wang2017ccsharp}. Metric-based approaches extract explicit features or metrics from source code to create vector representations, and code fragment similarity is computed using vector similarities. Nafi et al.~\cite{nafi2019clcdsa}, extracted nine metrics to detect cross-language clones. Learning-based approaches involve training machine learning models on existing datasets to perform clone detection. GraphCodeBERT was fine-tuned for the clone detection task~\cite{guo2020graphcodebert} using the BigCloneBench dataset~\cite{svajlenko2014towards}.

\subsection{Code duplication within GitHub}

SourcerCC~\cite{sajnani2016sourcerercc} was used by Lopes et al.~\cite{lopes2017dejavu} to perform an extensive study of code duplication within GitHub~\cite{lopes2017dejavu}. The study analyzed 4.5 million GitHub projects, encompassing 428M files written in Python, Java, and JavaScript. Key findings revealed that 70\% of code on GitHub consists of clones of previously created files, and a noteworthy amount of inter-project duplication exists (\textit{i.e}., files in one project can be found in another project).

Gharehyazie et al.\cite{gharehyazie2019cross} employed Deckard\cite{jiang2007deckard} to identify code clones within 8,599 GitHub projects. Employing a statistical and network approach, they concluded that cross-project cloning is a common practice across various granularities, ranging from several lines to entire projects. Additionally, they observed an onion model of cloning within GitHub, where the majority of clones originate from the same project, followed by projects within the same domain, and then from projects in different domains.

In an empirical study on the nature of code clones, Golubev and Bryksin~\cite{golubev2021nature} investigated a corpus of 23k open-source Java projects. Their findings indicated that, in Java, method-level duplication is more prevalent than file-level duplication. They also highlighted the common practice of copying/pasting code over the years of Java code existence.

Lastly, Yang et al.~\cite{yang2017stack} provided compelling evidence of code migration from Stack Overflow to GitHub, shedding light on one phenomenon that contributes to code duplication within GitHub. Utilizing SourcererCC, their study identified correspondences between 290M function definitions within GitHub and 1.9M Python snippets from Stack Overflow.
%maybe https://dl.acm.org/doi/abs/10.1145/3524610.3528390

%\subsection{ML for SE}
%TODO

\subsection{Code duplication and ML for code}

Allamanis~\cite{allamanis2019adverse} conducted a study on \emph{intra-dataset code duplication}, specifically examining the intersection between training and testing splits within code datasets and its implications for ML models. The study provided a set of best practices for gathering code corpora and assessing ML models on them. Subsequently, researchers, building upon this knowledge, have been aware of duplication issues and commonly implement deduplication strategies in their datasets~\cite{shi2022evaluation,husain2019codesearchnet,izadi2022codefill}. 
For example, Husain et al.\cite{husain2019codesearchnet} implemented a deduplication procedure before releasing the CSN dataset. Karmakar et al.\cite{karmakar2023jemma} incorporated deduplication as part of the preprocessing pipeline before releasing JEMMA, a large-scale, high-quality Java code corpus. Kocetkov et al.~\cite{kocetkov2022stack} released the deduplicated version of Stack, a massive 6TB source code corpus, demonstrating that pre-training code LLMs with a deduplicated version yields better results.

An inherent extension of Allamanis's work is the assessment of \emph{inter-dataset code duplication}, which poses a potential threat to the evaluation of ML models given the recent shift in learning paradigms (task specific training to pre-training/fine-tuning).


